Approach Towards Semi-Automated Certification for Low Criticality ML-Enabled Airborne Applications

As Machine Learning (ML) makes its way into aviation, ML enabled systems including low criticality systems require a reliable certification process to ensure safety and performance. Traditional standards, like DO 178C, which are used for critical software in aviation, do not fully cover the unique aspects of ML. This paper proposes a semi automated certification approach, specifically for low criticality ML systems, focusing on data and model validation, resilience assessment, and usability assurance while integrating manual and automated processes. Key aspects include structured classification to guide certification rigor on system attributes, an Assurance Profile that consolidates evaluation outcomes into a confidence measure the ML component, and methodologies for integrating human oversight into certification activities. Through a case study with a YOLOv8 based object detection system designed to classify military and civilian vehicles in real time for reconnaissance and surveillance aircraft, we show how this approach supports the certification of ML systems in low criticality airborne applications.

==> Sections/cert_ml_traditional.tex <==
% \begin{table*}[htbp]
% \caption{Certification Process Comparison: DO-178C vs. ML Systems}
% \centering
% \small
% \begin{tabular}{|p{3.5cm}|p{4cm}|p{4cm}|p{5cm}|}
% \hline
% Process &
%   DO-178C (Non-ML Software) &
%   ML Systems &
%   Additional Considerations for ML Systems \\ \hline
% \multirow{3}{*}{Planning Process} &
%   Flexible planning activities, minimal documentation &
%   Basic plans for data collection, model selection, and evaluation &
%   Clear development process needed despite flexibility \\ \cline{2-4}
%  &
%   Limited formality in defining software plans and standards &
%   Adaptable standards for data handling and model development &
%   Basic version control and data management practices required \\ \cline{2-4} 
%  &
%    &
%    &
%   Define and secure processes for user modifications to models or input data \\ \hline
% \multirow{2}{*}{Development Process} &
%   Requirements defined with focus on essential traceability &
%   Minimal requirements for data quality and model robustness &
%   Align rigor of requirements, design, and coding with system’s intended use and impact \\ \cline{2-4} 
%  &
%   Design and coding vary by system criticality &
%   Streamlined methods for model design and validation &
%    \\ \hline
% \multirow{2}{*}{Verification Process} &
%   Testing focused on functional correctness rather than exhaustive error removal &
%   Testing emphasizes model performance on relevant datasets &
%   Balance verification based on system criticality and error consequence risks \\ \cline{2-4} 
%  &
%   Simplified review and analysis procedures &
%   Basic methods for model interpretability and explainability (if needed) &
%    \\ \hline
% Configuration Management Process &
%   Basic configuration management (e.g., version control and change tracking) &
%   Streamlined version control and change management for ML models and datasets &
%   Essential traceability for model versions and data to ensure reproducibility and future updates \\ \hline
% \multirow{2}{*}{Quality Assurance Process} &
%   Limited quality assurance primarily for functionality and reliability &
%   Monitors model performance and potential drift with minimal rigor &
%   Allow less rigorous quality assurance but ensure model reliability and address ethical concerns \\ \cline{2-4} 
%  &
%    &
%    &
%   Ensure compliance with ethical and regulatory standards \\ \hline
% \end{tabular}
% \label{tab:ml_trad_cert_comparison}
% \end{table*}


% This section will provide a comparison between the certification process outlined in DO-178C for traditional software systems and the requirements needed for ML systems. The differences will be summarized in tables, highlighting areas where additional considerations are necessary for ML beyond what is specified in DO-178C. Additionally, a diagram will be included to contrast the certification workflows of traditional software systems and ML-enabled systems, emphasizing key distinctions in development, verification, and assurance activities.

% \input{Table/ml_trad_cert_process_comp}

Traditional certification standards like DO-178C have long provided a solid foundation to ensure software safety and reliability. However, with Machine Learning (ML) entering aviation, especially for low-criticality applications, we now need a new approach. As shown in Table \ref{tab:ml_trad_cert_comparison}, the certification process for ML systems differs across critical areas like verification and quality assurance, which in traditional software rely on code-level traceability and deterministic behavior. However, ML systems work in a probabilistic manner and are inherently adaptive. This shift requires certification to focus more on aspects like model performance, data quality, and interpretability, rather than strictly adhering to predefined requirements and static code paths.

The need to adapt certification practices is evident in the Air Sight case study, which focuses on an ML-based object detection system for airborne surveillance. Unlike traditional software, Air Sight processes complex, real-time visual data to aid decision-making in dynamic, low-criticality operational settings. This adaptability brings unique certification challenges: ensuring model robustness under varied and unpredictable conditions, handling data versioning, and sustaining model performance as new data continuously influence its behavior. Current certification frameworks like DO-178C are not equipped to address these aspects, leaving a gap in validating the ongoing accuracy and reliability of models that evolve and are re-trained on updated datasets.

This shift raises a fundamental question: How can we certify systems that learn and adapt continuously? Unlike traditional software, ML models, such as those in Air Sight, evolve and improve as they process new information, necessitating certification that considers elements not comprehensively addressed by current standards. Table \ref{tab:ml_trad_cert_comparison} provides a comparative overview, highlighting the unique needs of ML systems and revealing this gap in existing certification practices. ML models, rather than being fixed entities, require certification that accommodates continuous change and enables ongoing evaluation.

For instance, DO-178C emphasizes requirements-based testing for consistent, predictable results. However, ML systems like Air Sight require continuous validation across varied data distributions to ensure robustness and adaptability—something traditional standards do not yet fully address. This shift is not just a matter of updating procedures; it calls for certification to become a continuous process. As the EASA concept paper~\cite{easapaper} and studies by Dmitriev et al.~\cite{toolqualification} suggest, "Learning Assurance" and regular model performance monitoring are essential for the safe integration of ML systems in aviation. These methods help ensure that as Air Sight evolves, it remains within safe operational boundaries, adapting to new environments without compromising reliability.

The Air Sight case study shows why existing certification standards need to be updated to keep up with the demands of ML-based systems in aviation. It underlines the importance of building certification frameworks that allow for flexible validation, ongoing data management, and continuous monitoring to make sure ML systems like Air Sight stay both safe and adaptable in real-world use. 


==> Table/ml_trad_cert_process_comp.tex <==
\begin{table*}[htbp]
\caption{Certification Process Comparison: DO-178C vs. ML Systems}
\centering
\small
\begin{tabular}{|p{3.5cm}|p{4cm}|p{4cm}|p{5cm}|}
\hline
\textbf{Process} &
  \textbf{DO-178C (Non-ML Software Systems)} &
  \textbf{ML Systems} &
  \textbf{Additional Considerations for ML Systems} \\ \hline
\multirow{3}{*}{Planning Process} &
  Flexible planning activities, minimal documentation &
  Basic plans for data collection, model selection, and evaluation &
  Clear development process needed despite flexibility \\ \cline{2-4}
 &
  Limited formality in defining software plans and standards &
  Adaptable standards for data handling and model development &
  Basic version control and data management practices required \\ \cline{2-4} 
 &
   &
   &
  Define and secure processes for user modifications to models or input data \\ \hline
\multirow{2}{*}{Development Process} &
  Requirements defined with focus on essential traceability &
  Minimal requirements for data quality and model robustness &
  Align rigor of requirements, design, and coding with system’s intended use and impact \\ \cline{2-4} 
 &
  Design and coding vary by system criticality &
  Streamlined methods for model design and validation &
   \\ \hline
\multirow{2}{*}{Verification Process} &
  Testing focused on functional correctness rather than exhaustive error removal &
  Testing emphasizes model performance on relevant datasets &
  Balance verification based on system criticality and error consequence risks \\ \cline{2-4} 
 &
  Simplified review and analysis procedures &
  Basic methods for model interpretability and explainability (if needed) &
   \\ \hline
Configuration Management Process &
  Basic configuration management (e.g., version control and change tracking) &
  Streamlined version control and change management for ML models and datasets &
  Essential traceability for model versions and data to ensure reproducibility and future updates \\ \hline
\multirow{2}{*}{Quality Assurance Process} &
  Limited quality assurance primarily for functionality and reliability &
  Monitors model performance and potential drift with minimal rigor &
  Allow less rigorous quality assurance but ensure model reliability and address ethical concerns \\ \cline{2-4} 
 &
   &
   &
  Ensure compliance with ethical and regulatory standards \\ \hline
\end{tabular}
\label{tab:ml_trad_cert_comparison}
\end{table*}

==> cuts.tex <==
\subsection{Certification Levels Based on Criticality}
The certification process follows the DO-178C-inspired framework, defining certification levels based on the severity of system failure:

\begin{itemize}
    \item \textbf{Level A}: Catastrophic (Failure could cause a crash)
    \item \textbf{Level B}: Hazardous (Failure significantly impacts safety)
    \item \textbf{Level C}: Major (Failure impacts safety but is manageable)
    \item \textbf{Level D}: Minor (Failure has minimal operational impact)
    \item \textbf{Level E}: No Effect (Failure has no safety impact)
\end{itemize}

For low-criticality applications (Levels C, D, E), the focus is less on stringent robustness checks and more on ensuring the system is operationally safe.

\subsection{Core Evaluation Categories and Dynamic Weighting}
Each category in the evaluation framework is weighted differently depending on the criticality level. The weights represent the relative importance of each category for certification at that level.

\subsubsection{Data Integrity}
Ensuring data quality is crucial for robust training and inference:
\begin{itemize}
    \item \textbf{Checks}: Outliers (image and label properties), label-property correlation, class balance, missing data, and anomalies.
    \item \textbf{Weight by Criticality}:
    \begin{itemize}
        \item \textbf{Level A/B}: 35\%
        \item \textbf{Level C}: 30\%
        \item \textbf{Level D/E}: 25\%
    \end{itemize}
\end{itemize}

\subsubsection{Train-Test Evaluation}
This category assesses the consistency and generalizability of the model across the dataset splits:
\begin{itemize}
    \item \textbf{Checks}: Data drift, feature consistency, and predictive power score (PPS) stability between training and testing sets.
    \item \textbf{Weight by Criticality}:
    \begin{itemize}
        \item \textbf{Level A/B}: 30\%
        \item \textbf{Level C}:25\%
        \item \textbf{Level D/E}: 20\%
    \end{itemize}
\end{itemize}

\subsubsection{Model Performance}
Model performance is key to ensuring the system can reliably perform its task, particularly for object detection models:
\begin{itemize}
    \item \textbf{Checks}: mAP, false positives/negatives, edge case handling (e.g., occlusion, lighting variations), robustness to noise, and adversarial scenarios.
    \item \textbf{Weight by Criticality}:
    \begin{itemize}
        \item \textbf{Level A/B}: 40\%
        \item \textbf{Level C}:35\%
        \item \textbf{Level D/E}: 30\%
    \end{itemize}
\end{itemize}

\subsubsection{Resource Utilization}
For real-time airborne systems, resource efficiency (e.g., latency and memory usage) is crucial, particularly for embedded hardware:
\begin{itemize}
    \item \textbf{Checks}: Inference latency, GPU/CPU memory usage, and computational load under real-time conditions.
    \item \textbf{Weight by Criticality}:
    \begin{itemize}
        \item \textbf{Level A/B}: 10\%
        \item \textbf{Level C}:10\%
        \item \textbf{Level D/E}: 25\%
    \end{itemize}
\end{itemize}

\subsection{Certification Scoring and Confidence Levels}
The certification process uses a scoring mechanism to assess overall readiness based on the weighted category scores. Adjustments to the score thresholds are made based on the system's criticality level.

\subsubsection{Scoring Breakdown}
\begin{itemize}
    \item \textbf{Category Scores}: Each check within a category is scored from 0 to 1 based on specific criteria.
    \item \textbf{Weighted Category Scores}: The final category scores are calculated based on the criticality-adjusted weights.
    \item \textbf{Final Score}: A weighted average of the category scores gives the overall certification score.
\end{itemize}

\textbf{Criticality-Based Thresholds}
\begin{itemize}
    \item \textbf{Low Criticality (Level C/D/E)}: 
    \begin{itemize}
        \item \textbf{Certified with High Confidence}: \textgreater75\%
        \item \textbf{Certified with Moderate Confidence}: 60-75\%
        \item \textbf{Low Confidence/Not Certified}: $<$60\%
    \end{itemize}
    \item \textbf{High Criticality (Level A/B)}: 
    \begin{itemize}
        \item \textbf{Certified with High Confidence}: \textgreater85\%
        \item \textbf{Certified with Moderate Confidence}: 70-85\%
        \item \textbf{Low Confidence/Not Certified}: $<$70\%
    \end{itemize}
\end{itemize}

\subsection{Semi-Automated Certification Tool}
The tool automates many of the key checks and evaluations. It integrates modules from the DeepChecks library and custom-built components for performance and resource evaluations, making the certification process more scalable and systematic.

\subsubsection{Inputs}
    \begin{itemize}
        \item Object detection model (e.g., YOLOv8)
        \item Dataset (training and testing)
        \item Intended application level (criticality level)
    \end{itemize}
    
\subsubsection{Processes}
    \begin{itemize}
        \item \textbf{Data Integrity}: Runs outlier detection, anomaly checks, and label-property correlation analysis.
        \item \textbf{Train-Test Evaluation}: Evaluates data drift and feature consistency between training and test sets, including PPS.
        \item \textbf{Model Performance}: Tests for mAP, false positives/negatives, edge case handling, and robustness to noise.
        \item \textbf{Resource Utilization}: Measures inference latency, memory usage, and computational load.
    \end{itemize}
    
\subsubsection{Outputs}
    \begin{itemize}
        \item Scores for each evaluation category based on the criticality-adjusted weights.
        \item Final certification score with confidence level.
        \item Detailed report including key metrics, visualizations, and failure case analysis.
    \end{itemize}





    % The introduction of ML-based systems in aviation, as illustrated through the Air Sight case study in Section~\ref{sec:case_study} and~\ref{sec:cert_ml_traditional}, highlights the limitation of traditional certification standards like DO-178C~\cite{178C}. These standards, which emphasize static code traceability and deterministic behaviour of software systems, fall short in accomodating the dynamic, data-driven and adaptive nature of MLS. Our proposed framework addresses this gap by prioritizing continuous model performance evaluation, data quality management and adaptability assurance, essential for certifying systems that learn and evolve. By advancing certification practices to include "Learning Assurance"~\cite{easapaper} and ongoing monitoring, this framework lays the foundation for the safe integration of MLS in aviation, ensuring they remain robust and reliable in real-world, low-criticality applications.The integration of ML-based systems into aviation introduces new certification challenges, as seen with the Air Sight case study. Traditional certification standards, such as DO-178C, which emphasize static code traceability and deterministic behavior, lack the adaptability needed for certifying data-driven, dynamically evolving MLS. Our proposed semi-automated certification framework addresses these gaps by emphasizing continuous model performance evaluation, data quality management, and resilience in varied operational contexts.

% By incorporating "Learning Assurance" and post-deployment monitoring, this framework ensures that ML systems remain compliant, reliable, and robust in low-criticality aviation applications. This approach allows ML-enabled systems to evolve safely and effectively, meeting regulatory and operational standards. This certification model advances the field by aligning traditional safety requirements with the flexibility and adaptability that ML-based systems demand, supporting their safe and effective integration into aviation.
